Invariant Pretraining for Robust Code Representations

Encoder-based code representation models remain widely deployed for discriminative tasks such as clone detection and code classification, where their small size and low inference cost are decisive. Their robustness, however, is fragile: under invariant programs, semantically equivalent code written in different syntactic forms, learned representations degrade substantially even though program behavior is unchanged. We present an empirical study of this robustness gap across four encoder baselines, two downstream tasks, and four datasets, together with a minimal code-only continued pretraining recipe that closes much of it. Our method, invariant pretraining (InvPT), applies semantic-preserving transformations to the corpus and combines masked language modeling with multi-positive supervised contrastive learning that treats all augmentations of the same source function as positives, mixing self-contrast pairs (same code, different masks) with invariant-contrast pairs (transformed code) for positives of varying difficulty. Unlike prior contrastive code encoders, InvPT does not require paired natural-language data. Across our evaluation, InvPT improves robustness on transformed test sets by up to 11 percentage points on clone detection and 19 on code classification while matching or improving standard accuracy, and our ablations isolate multi-positive invariant contrast as the main source of the gains. Our aim is not a new objective but a careful measurement of where encoder robustness breaks and how far a simple, code-only recipe can recover it.

==> src/attacks.tex <==
\section{Invariant Pretraining Under Attacks}

==> src/background.tex <==
\section{Background}

==> src/ethics.tex <==
\section*{Ethics Statement}

Our method improves the robustness of code representation models through semantics-preserving transformations and contrastive learning.
Improved semantic understanding of programs facilitates various downstream tasks such as clone detection and code classification, which further support detecting code plagiarism and identifying functionally similar programs.
All datasets used in this work (CodeSearchNet, POJ104, CodeNet) are publicly available under permissive licenses.
We do not collect new data from human subjects and do not foresee direct negative societal impact from this research.


==> tables/classification+T.tex <==
\begin{tabular}{l N@{}l N@{}l N@{}l N@{}l}
	\toprule
	Model            & \multicolumn{2}{c}{Java250} & \multicolumn{2}{c}{Python800} & \multicolumn{2}{c}{C++1400} & \multicolumn{2}{c}{POJ104}                                                                 \\
	\midrule
	CodeBERT         & 65.81                       &                               & 63.26                       &                            & 39.92           &             & 50.97           &             \\
	GraphCodeBERT    & 67.51                       &                               & 78.52                       &                            & 41.52           &             & 52.03           &             \\
	\contrabc        & 67.33                       &                               & 72.61                       &                            & 41.46           &             & 51.19           &             \\
	\contrabg        & 68.57                       &                               & 78.59                       &                            & 41.23           &             & 50.38           &             \\
	\lightmidrule
	InvCodeBERT      & 70.10                       & \rimp{+6.5}                   & 82.42                       & \rimp{+30.3}               & 43.69           & \rimp{+9.4} & 53.67           & \rimp{+5.3} \\
	InvGraphCodeBERT & 71.30                       & \rimp{+5.6}                   & \bfseries 84.60             & \rimp{+7.7}                & \bfseries 44.23 & \rimp{+6.5} & 52.66           & \rimp{+1.2} \\
	InvContraBERT\_C & 71.35                       & \rimp{+6.0}                   & 83.28                       & \rimp{+14.7}               & 42.51           & \rimp{+2.5} & 53.24           & \rimp{+4.0} \\
	InvContraBERT\_G & \bfseries 71.48             & \rimp{+4.2}                   & 83.42                       & \rimp{+6.1}                & 42.88           & \rimp{+4.0} & \bfseries 53.74 & \rimp{+6.7} \\
	\bottomrule
\end{tabular}


==> tables/classification.tex <==
\begin{tabular}{l N@{}l N@{}l N@{}l N@{}l}
	\toprule
	Model            & \multicolumn{2}{c}{Java250} & \multicolumn{2}{c}{Python800} & \multicolumn{2}{c}{C++1400} & \multicolumn{2}{c}{POJ104}                                             \\
	\midrule
	CodeBERT         & 97.80                       &                               & 98.92                       &                            & 89.63 &             & 98.51 &             \\
	GraphCodeBERT    & 97.97                       &                               & 99.06                       &                            & 89.70 &             & 98.68 &             \\
	\contrabc        & 97.90                       &                               & 98.89                       &                            & 89.54 &             & 98.48 &             \\
	\contrabg        & 98.15                       &                               & 99.10                       &                            & 89.53 &             & 98.63 &             \\
	\lightmidrule
	InvCodeBERT      & 98.16                       & \rimp{+0.4}                   & 99.00                       & \rimp{+0.1}                & 89.94 & \rimp{+0.3} & 98.63 & \rimp{+0.1} \\
	InvGraphCodeBERT & 98.08                       & \rimp{+0.1}                   & 99.09                       & \rimp{+0.0}                & 90.00 & \rimp{+0.3} & 98.54 & \rimp{-0.1} \\
	InvContraBERT\_C & 98.07                       & \rimp{+0.2}                   & 98.95                       & \rimp{+0.1}                & 89.87 & \rimp{+0.4} & 98.72 & \rimp{+0.2} \\
	InvContraBERT\_G & 98.21                       & \rimp{+0.1}                   & 99.11                       & \rimp{+0.0}                & 89.71 & \rimp{+0.2} & 98.73 & \rimp{+0.1} \\
	\bottomrule
\end{tabular}

==> tables/clone+T.tex <==
\begin{tabular}{l N@{}l N@{}l N@{}l N@{}l}
	\toprule
	Model            & \multicolumn{2}{c}{Java250} & \multicolumn{2}{c}{Python800} & \multicolumn{2}{c}{C++1400} & \multicolumn{2}{c}{POJ104}                                                                   \\
	\midrule
	CodeBERT         & 51.16                       &                               & 62.17                       &                            & 25.59           &              & 55.96           &              \\
	GraphCodeBERT    & 53.52                       &                               & 65.89                       &                            & 30.26           &              & 58.63           &              \\
	\contrabc        & 49.64                       &                               & 63.41                       &                            & 27.09           &              & 62.76           &              \\
	\contrabg        & 53.79                       &                               & 65.98                       &                            & 29.11           &              & 64.20           &              \\
	CodeSage         & 25.92                       &                               & 25.89                       &                            & 21.33           &              & 52.87           &              \\
	ModernBERT       & 41.06                       &                               & 52.85                       &                            & 24.66           &              & 52.86           &              \\
	\lightmidrule
	InvCodeBERT      & 59.27                       & \rimp{+15.9}                  & 70.55                       & \rimp{+13.5}               & 31.43           & \rimp{+22.8} & 62.03           & \rimp{+10.8} \\
	InvGraphCodeBERT & \bfseries 62.30             & \rimp{+16.4}                  & 73.91                       & \rimp{+12.2}               & \bfseries 33.68 & \rimp{+11.3} & 67.32           & \rimp{+14.8} \\
	InvContraBERT\_C & 60.68                       & \rimp{+22.2}                  & 74.34                       & \rimp{+17.2}               & 32.07           & \rimp{+18.4} & 63.53           & \rimp{+1.2}  \\
	InvContraBERT\_G & 62.24                       & \rimp{+15.7}                  & \bfseries 74.60             & \rimp{+13.1}               & 33.10           & \rimp{+13.7} & \bfseries 68.63 & \rimp{+6.9}  \\
	\bottomrule
\end{tabular}

==> tables/clone.tex <==
\begin{tabular}{l N@{}l N@{}l N@{}l N@{}l}
	\toprule
	Model            & \multicolumn{2}{c}{Java250} & \multicolumn{2}{c}{Python800} & \multicolumn{2}{c}{C++1400} & \multicolumn{2}{c}{POJ104}                                                                 \\
	\midrule
	CodeBERT         & 77.28                       &                               & 83.71                       &                            & 56.21           &             & 85.47           &             \\
	GraphCodeBERT    & 82.15                       &                               & 86.06                       &                            & 58.76           &             & 84.09           &             \\
	\contrabc        & 82.19                       &                               & 85.60                       &                            & 57.65           &             & 89.58           &             \\
	\contrabg        & 83.47                       &                               & 85.97                       &                            & 59.15           &             & 90.80           &             \\
	CodeSage         & 72.43                       &                               & 61.11                       &                            & 51.53           &             & 78.20           &             \\
	ModernBERT       & 80.51                       &                               & 83.16                       &                            & 59.05           &             & 88.22           &             \\
	\lightmidrule
	InvCodeBERT      & 82.44                       & \rimp{+6.7}                   & 85.63                       & \rimp{+2.3}                & 57.80           & \rimp{+2.8} & 88.81           & \rimp{+3.9} \\
	InvGraphCodeBERT & 84.41                       & \rimp{+2.8}                   & \bfseries 86.73             & \rimp{+0.8}                & \bfseries 59.23 & \rimp{+0.8} & 90.66           & \rimp{+7.8} \\
	InvContraBERT\_C & 82.63                       & \rimp{+0.5}                   & 86.16                       & \rimp{+0.7}                & 58.09           & \rimp{+0.8} & 89.28           & \rimp{-0.3} \\
	InvContraBERT\_G & \bfseries 84.53             & \rimp{+1.3}                   & 86.34                       & \rimp{+0.4}                & 59.23           & \rimp{+0.1} & \bfseries 91.25 & \rimp{+0.5} \\
	\bottomrule
\end{tabular}
